Novelty-Driven Binary Particle Swarm Optimisation for Truss Optimisation Problems

Topology optimisation of trusses can be formulated as a combinatorial and multi-modal problem in which locating distinct optimal designs allows practitioners to choose the best design based on their preferences. Bilevel optimisation has been successfully applied to truss optimisation to consider topology and sizing in upper and lower levels, respectively. We introduce exact enumeration to rigorously analyse the topology search space and remove randomness for small problems. We also propose novelty-driven binary particle swarm optimisation for bigger problems to discover new designs at the upper level by maximising novelty. For the lower level, we employ a reliable evolutionary optimiser to tackle the layout configuration aspect of the problem. We consider truss optimisation problem instances where designers need to select the size of bars from a discrete set with respect to practice code constraints. Our experimental investigations show that our approach outperforms the current state-of-the-art methods and it obtains multiple high-quality solutions.

==> tables/table_10.tex <==
\begin{tabular}{@{}lllllllll@{}}
\toprule
% A : in\textsuperscript{2}
& \cite{Li2009}  & \cite{HoHuu2016} & \cite{Cheng2016} & \cite{Fenton2014} & \cite{Khayyam2020} & \multicolumn{3}{c}{This Study} \\
\midrule
               &       &       &                  &           &                                 & (a)       & (b)       & (c)       \\
% \cmidrule{7-9}
% $A_1$               & 30      & 33.5       & 33.5                 & 29.5          & 30          & 30       & 30       & 30       \\
% $A_2$               & 1.62    & 1.62       & 1.62                  & -             & -           & -        & 1.62     & -        \\
% $A_3$               & 22.9    & 22.9       & 22.9                & 23.6          & 22          & 22       & 22       & 22       \\
% $A_4$               & 13.5    & 14.2       & 14.2                 & 16.8          & 13.9        & 13.5     & 14.2     & 14.2     \\
% $A_5$               & 1.62    & 1.62       & 1.62                  & -             & -           & -        & -        & -        \\
% $A_6$              & 1.62    & 1.62       & 1.62                  & -             & -           & -        & 1.62     & 1.62     \\
% $A_7$               & 7.97    & 7.97       & 7.97                  & 6.1           & 7.22        & 7.22     & 7.22     & 7.22     \\
% $A_8$               & 26.5    & 22.9       & 22.9                 & 21            & 22          & 22       & 22       & 22       \\
% $A_9$               & 22      & 22         & 22                  & 22.8          & 22          & 22       & 22       & 22       \\
% $A_{10}$              & 1.8     & 1.62       & 1.62                 & -             & -           & -        & -        & 1.62     \\
\textbf{\shortstack{Best weight (lb)}} & 5531.98 & 5490.74    & 5490.74       & 5056.88       & 4980.10     & 4965.7   & 5107.5   & 5131.7  \\
\bottomrule
\end{tabular}

% % A                  & HPSO    & aeDE       & HHS       & GE             & DO-GE        & Khayyam    & AA       & BB       & CC       \\

==> tables/table_25-1.tex <==
\begin{tabular}{lllllll}
\toprule
% A : in\textsuperscript{2}
& \cite{Rajeev1992} & \cite{HoHuu2016}  & \cite{Cheng2016} & \multicolumn{3}{c}{This Study} \\
\midrule
&&&       & (a)        & (b)      & (c)       \\
\cmidrule{5-7}
% $A_1$               & 0.1        & 0.1        & 0.1       & -        & 0.1       & -       \\
% $A_2 - A_5$              & 1.8        & 0.3        & 0.3       & 0.3      & 0.3       & 0.5     \\
% $A_6 - A_9$               & 2.3        & 3.4        & 3.4       & 3.4      & 3.4       & 3.4     \\
% $A_{10} - A_{11}$               & 0.2        & 0.1        & 0.1       &-        & -         & 0.1     \\
% $A_{12} - A_{13}$               & 0.1        & 2.1        & 2.1       & 2.1      & 2.1       & 1.9     \\
% $A_{14} - A_{17}$               & 0.8        & 1          & 1         & 1        & 1         & 0.9     \\
% $A_{18} - A_{21}$               & 1.8        & 0.5        & 0.5       & 0.5      & 0.5       & 0.5     \\
% $A_{22} - A_{25}$              & 3          & 3.4        & 3.4       & 3.4      & 3.4       & 3.4     \\
\textbf{Best weight (lb)} & 546.01     & 484.85     & 484.85    & 482.6    & 483.35    & 484.3  \\
\bottomrule
\end{tabular}

==> tables/table_25-2.tex <==
\begin{tabular}{llllll}
\toprule
% A : in\textsuperscript{2}
& \cite{Lee2005} & \cite{Li2009}  & \multicolumn{3}{c}{This Study} \\
\midrule
&&       & (a)        & (b)      & (c)       \\
\cmidrule{4-6}
% $A_1$             & 0.307   & 0.111  & -        & 0.111    & -        \\
% $A_2 - A_5$       & 1.99    & 2.13   & 2.13     & 2.13     & 2.13     \\
% $A_6 - A_9$       & 3.13    & 2.88   & 2.88     & 2.88     & 2.88     \\
% $A_{10} - A_{11}$ & 0.111   & 0.111  & -        & -        & -        \\
% $A_{12} - A_{13}$ & 0.141   & 0.111  & -        & -        & 0.111    \\
% $A_{14} - A_{17}$ & 0.766   & 0.766  & 0.766    & 0.766    & 0.766    \\
% $A_{18} - A_{21}$ & 1.62    & 1.62   & 1.62     & 1.62     & 1.62     \\
% $A_{22} - A_{25}$ & 2.62    & 2.62   & 2.62     & 2.62     & 2.62     \\
\textbf{Best weight (lb)}  & 556.43  & 551.14 & 546.97   & 547.81   & 548.64 \\
\bottomrule
\end{tabular}


==> tables/table_25.tex <==
\begin{tabular}{@{}llllllllllllll@{}}
\toprule
& \multicolumn{6}{c}{\textbf{Case 1}} & \multicolumn{6}{c}{\textbf{Case 2}} \\
\cmidrule{2-7} \cmidrule{9-13}
% A : in\textsuperscript{2}
& \cite{Rajeev1992} & \cite{HoHuu2016}  & \cite{Cheng2016} & \multicolumn{3}{c}{\textbf{This Study}} && \cite{Lee2005} & \cite{Li2009}  & \multicolumn{3}{c}{\textbf{This Study}} \\
\midrule
&&&& (a)        & (b)      & (c) &&&& (a)        & (b)      & (c)  \\
\cmidrule{5-7} \cmidrule{11-13}
% $A_1$             & 0.1    & 0.1    & 0.1    & -        & 0.1       & -       && 0.307  & 0.111  & -        & 0.111    & -        \\
% $A_2 - A_5$       & 1.8    & 0.3    & 0.3    & 0.3      & 0.3       & 0.5     && 1.99   & 2.13   & 2.13     & 2.13     & 2.13     \\
% $A_6 - A_9$       & 2.3    & 3.4    & 3.4    & 3.4      & 3.4       & 3.4     && 3.13   & 2.88   & 2.88     & 2.88     & 2.88     \\
% $A_{10} - A_{11}$ & 0.2    & 0.1    & 0.1    & -        & -         & 0.1     && 0.111  & 0.111  & -        & -        & -        \\
% $A_{12} - A_{13}$ & 0.1    & 2.1    & 2.1    & 2.1      & 2.1       & 1.9     && 0.141  & 0.111  & -        & -        & 0.111    \\
% $A_{14} - A_{17}$ & 0.8    & 1      & 1      & 1        & 1         & 0.9     && 0.766  & 0.766  & 0.766    & 0.766    & 0.766    \\
% $A_{18} - A_{21}$ & 1.8    & 0.5    & 0.5    & 0.5      & 0.5       & 0.5     && 1.62   & 1.62   & 1.62     & 1.62     & 1.62     \\
% $A_{22} - A_{25}$ & 3      & 3.4    & 3.4    & 3.4      & 3.4       & 3.4     && 2.62   & 2.62   & 2.62     & 2.62     & 2.62     \\
\textbf{Best weight} (lb)  & 546.01 & 484.85 & 484.85 & 482.6    & 483.35    & 484.3   && 556.43 & 551.14 & 546.97   & 547.81   & 548.64  \\
\bottomrule
\end{tabular}

==> tables/table_25_1_new.tex <==
\begin{tabular}{llllllll}
\toprule
% A : in\textsuperscript{2}
& \cite{Rajeev1992} & \multicolumn{3}{c}{\cite{HoHuu2016}, \cite{Cheng2016}, \cite{Degertekin2019}} & \multicolumn{3}{c}{This Study} \\
\midrule
&&&       && (a)        & (b)      & (c)       \\
\cmidrule{6-8}
\textbf{Best weight (lb)} & 546.01     & \multicolumn{3}{c}{484.85} & 482.6    & 483.35    & 484.3  \\
\bottomrule
\end{tabular}

==> tables/table_25_2_new.tex <==
\begin{tabular}{lllllll}
\toprule
% A : in\textsuperscript{2}
& \cite{Lee2005} & \multicolumn{2}{l}{\cite{Li2009}, \cite{Degertekin2019}} & \multicolumn{3}{c}{This Study} \\
\midrule
&&       && (a)        & (b)      & (c)       \\
\cmidrule{5-7}
\textbf{Best weight (lb)}  & 556.43  & \multicolumn{2}{c}{551.14} & 546.97   & 547.81   & 548.64 \\
\bottomrule
\end{tabular}



% $A_1$             & 0.307   & 0.111  & -        & 0.111    & -        \\
% $A_2 - A_5$       & 1.99    & 2.13   & 2.13     & 2.13     & 2.13     \\
% $A_6 - A_9$       & 3.13    & 2.88   & 2.88     & 2.88     & 2.88     \\
% $A_{10} - A_{11}$ & 0.111   & 0.111  & -        & -        & -        \\
% $A_{12} - A_{13}$ & 0.141   & 0.111  & -        & -        & 0.111    \\
% $A_{14} - A_{17}$ & 0.766   & 0.766  & 0.766    & 0.766    & 0.766    \\
% $A_{18} - A_{21}$ & 1.62    & 1.62   & 1.62     & 1.62     & 1.62     \\
% $A_{22} - A_{25}$ & 2.62    & 2.62   & 2.62     & 2.62     & 2.62     \\

==> tables/table_52.tex <==
\begin{tabular}{llllllllll}
\toprule
% A : mm\textsuperscript{2}
& \cite{Wu1995}   & \cite{Lee2005}  & \cite{Li2009}   & \cite{Kaveh2009} & \cite{HoHuu2016} & \cite{Cheng2016} & \multicolumn{3}{c}{This Study} \\
\midrule
&&&&&& & (a) & (b) & (c) \\
\cmidrule{8-10}
% $A_{1} - A_{4}$            & 4658.055 & 4658.055 & 4658.055 & 4658.055  & 4658.055   & 4658.055  & 5141.925 & 4658.055 & 4658.055 \\
% $A_{5} - A_{10}$           & 1161.288 & 1161.288 & 1161.288 & 1161.288  & 1161.288   & 1161.288  & 939.998  & 1045.159 & 1008.385 \\
% $A_{11} - A_{13}$            & 645.160  & 506.451  & 363.225  & 494.193   & 494.193    & 494.193   & -    & -    & -    \\
% $A_{14} - A_{17}$             & 3303.219 & 3303.219 & 3303.219 & 3303.219  & 3303.219   & 3303.219  & 3703.218 & 3703.218 & 3703.218 \\
% $A_{18} - A_{23}$           & 1045.159 & 940.000  & 940.000  & 1008.385  & 939.998    & 940.000   & 792.256  & 939.998  & 1008.385 \\
% $A_{24} - A_{26}$            & 494.193  & 494.193  & 494.193  & 285.161   & 494.193    & 494.193   & -    & -    & 198.064  \\
% $A_{27} - A_{30}$             & 2477.414 & 2290.318 & 2238.705 & 2290.318  & 2283.705   & 2238.705  & 2477.414 & 2477.414 & 2341.931 \\
% $A_{31} - A_{36}$            & 1045.159 & 1008.385 & 1008.385 & 1008.385  & 1008.385   & 1008.385  & 939.998  & 1008.385 & 939.998  \\
% $A_{37} - A_{39}$            & 285.161  & 363.225  & 388.386  & 388.386   & 494.193    & 494.193   & -    & 198.064  & 285.161  \\
% $A_{40} - A_{43}$           & 1696.771 & 1535.481 & 1283.868 & 1283.868  & 1283.868   & 1283.868  & 1535.481 & 1535.481 & 1535.481 \\
% $A_{44} - A_{49}$            & 1045.159 & 1045.159 & 1161.288 & 1161.288  & 1161.288   & 1161.288  & 1045.159 & 1008.385 & 1008.385 \\
% $A_{50} - A_{52}$           & 641.289  & 506.451  & 792.256  & 506.451   & 494.193    & 494.193   & 363.225  & 494.193  & 388.386  \\
\textbf{Best weight (kg)} & 1970.140 & 1906.760 & 1905.500 & 1904.830  & 1902.610   & 1902.610  & 1862.000  & 1880.300  & 1869.7 \\
\bottomrule
\end{tabular}

==> tables/table_72.tex <==
\begin{tabular}{lllllll}
\toprule
% A : in.\textsuperscript{2}
& \cite{Wu1995} & \cite{Lee2005} & \cite{Cheng2016} & \multicolumn{3}{c}{This Study} \\
\midrule
&&& & (a) & (b) & (c)\\
\cmidrule{5-7}
% $A_{1} - A_{4}$                               & 1.5                            & 1.9                             & 1.9                               & 2        & 2        & 1.9      \\
% $A_{5} - A_{12}$                            & 0.7                            & 0.5                             & 0.5                               & 0.5      & 0.5      & 0.5      \\
% $A_{13} - A_{16}$                           & 0.1                            & 0.1                             & 0.1                               & -        & -        & -        \\
% $A_{17} - A_{18}$                           & 0.1                            & 0.1                             & 0.1                               & -        & -        & -        \\
% $A_{19} - A_{22}$                           & 1.3                            & 1.4                             & 1.4                               & 1.4      & 1.3      & 1.3      \\
% $A_{23} - A_{30}$                           & 0.5                            & 0.6                             & 0.5                               & 0.6      & 0.5      & 0.5      \\
% $A_{31} - A_{34}$                           & 0.2                            & 0.1                             & 0.1                               & -        & -        & -        \\
% $A_{35} - A_{36}$                           & 0.1                            & 0.1                             & 0.1                               & -        & -        & 0.1      \\
% $A_{37} - A_{40}$                           & 0.5                            & 0.6                             & 0.5                               & 0.5      & 0.5      & 0.5      \\
% $A_{41} - A_{48}$                           & 0.5                            & 0.5                             & 0.5                               & 0.5      & 0.5      & 0.6      \\
% $A_{49} - A_{52}$                           & 0.1                            & 0.1                             & 0.1                               & -        & -        & -        \\
% $A_{53} - A_{54}$                           & 0.2                            & 0.1                             & 0.1                               & -        & 0.1      & -       \\
% $A_{55} - A_{58}$                           & 0.2                            & 0.2                             & 0.2                               & 0.2      & 0.2      & 0.2      \\
% $A_{59} - A_{66}$                           & 0.5                            & 0.5                             & 0.6                               & 0.5      & 0.6      & 0.5      \\
% $A_{67} - A_{70}$                           & 0.5                            & 0.4                             & 0.4                               & 0.5      & 0.5      & 0.5      \\
% $A_{71} - A_{72}$                           & 0.7                            & 0.6                             & 0.6                               & 0.6      & 0.6      & 0.7      \\
\textbf{Best Weight (lb)}                            & 400.66                         & 387.94                          & 385.54                            & 368.16   & 369.15   & 370.15   \\
\bottomrule
\end{tabular}

==> tables/table_data.tex <==
\begin{tabular}{llllll}
\toprule
                                         & 25-bar   & 10-bar & 52-bar  & 15-bar  & 72-bar   \\
\midrule                                         
Number of nodes $(n)$                    & 10       & 6      & 20      & 8       & 20       \\
Number of bars $(m)$                     & 25       & 10     & 52      & 15      & 72       \\
Length of topology & 8        & 10     & 12      & 15      & 16       \\
design variable ($m$) & & & & & \\
 Symmetry                                & Yes      & No     & Yes     & No      & Yes      \\
% Allowable stress                         & 40 ksi   & 25 ksi & 180 Mpa & 120 Mpa & 25 ksi   \\
% Allowable displacement                   & 0.35 in. & 2 in.  & -       & 10 mm   & 0.25 in. \\
\bottomrule
\end{tabular}
